Collision-Aware Fast Simulation for Soft Robots by Optimization-Based Geometric Computing

Soft robots can safely interact with environments because of their mechanical compliance. Self-collision is also employed in the modern design of soft robots to enhance their performance during different tasks. However, developing an efficient and reliable simulator that can handle the collision response well, is still a challenging task in the research of soft robotics. This paper presents a collision-aware simulator based on geometric optimization, in which we develop a highly efficient and realistic collision checking / response model incorporating a hyperelastic material property. Both actuated deformation and collision response for soft robots are formulated as geometry-based objectives. The collision-free body of a soft robot can be obtained by minimizing the geometry-based objective function. Unlike the FEA-based physical simulation, the proposed pipeline performs a much lower computational cost. Moreover, adaptive remeshing is applied to achieve the improvement of the convergence when dealing with soft robots that have large volume variations. Experimental tests are conducted on different soft robots to verify the performance of our approach.

==> tex/secIntroduction.tex <==
\section{Introduction}
\label{sec:intro}

\IEEEPARstart{I}{n} robotic research, control robot manipulators for the precise and efficient grasping motion is a fundamental problem that has been widely studied for industrial automation. A traditional rigid-joint robotic arm solution usually realizes the grasping task by moving the end-effector (i.e. gripper) to desired position and apply grasp motion to pick the object~\cite{Saxena06_NIPS}. In recent years, with the development of both the design aspects and the fabrication process, robots with continuum bodies made of soft material have proven their capability of achieving tasks in positioning and grasping~\cite{Glick18_RAL, Marchese14_IROS}. As the soft material made manipulator and gripper are safer when interacting with environments, they have the adaptability to grasp soft objects with unknown shapes~\cite{Langowski20_sciRobot}. In this sense, soft grippers come up with another robotic grasping solutions and have already been commercialized in industry (e.g. FESTO bio-hand and Soft Robotics Inc.). 

However, the manipulator made with soft body have infinite \textit{degrees-of-freedoms} (DoFs) in configuration space (defined by~\cite{}), which invite a high complexity in building a precise kinematics model and control theory that involves collision checking. When interact with environment contains obstacles, tremendous effort on predict the whole body shape for collision checking is required for motion planning. On the other hand, soft robots system can be highly redundant (the actuator numbers higher than end-effector configuration dimension), which brings a multi-solution in configuration can be detected for the same position in task space~\cite{}. This brings more challenge in solving the actuation constraints in planning the motion. The manipulators is commonly used in achieve high-level task such pick-and-place objects or detect confined area. Where a hieletci-level task can be detected. To solve this problem, we need to 

\guoxin{Update 08-13, why we need collision avidance for soft robot? this based on the application. For the task such as pick-and-place soft object in non-critical environment, the restriction for collision checking can be relaxed. However for application such as surgrical manipulation, any undesirable contact between tools and organs can have severe consequences. Therefore this case the accurate collisio-free path planning is essential for these applications. // this is also the reason why we train the distance field and can control the ability to control the collision possibility to the obstacle.}

As a high-level control problem, motion planning for grasping (i.e. pick-and-place task) also requires a proper formulation of the task.

The difficulties of building a effective motion planning algorithm for soft manipulators to achieve task in restricted environment comes from different aspects. Firstly, it's not 

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{fig/illustration.jpg}
    \caption{Illustration of difference between (a) rigid robotic arm grasping and (b) soft manipulator grasping. \guoxin{figure replaced later.}} 
    \label{fig:illustration}
\end{figure}

\subsection{Related Work}

\guoxin{ --- Related work on rigid robot grasping task}

For the motion planning of rigid robot grasping task, a multi-level optimization scheme is recently presented in~\cite{Zimmermann20_RAL}. However they didn't consider the redundancy of the system in the control loop.

\guoxin{ --- Related work on soft robot motion planning / collision avoidance}

\guoxin{Here should also includes the analytical-based control method, and make clear why numerical-based optimization is important.}

\guoxin{Also mention most case the interact of soft robot is conducted in reference. However a proper motion planning is still necessary for a initial guess, particularly for narrow region with obstacles.}
.

.

.
%By building up the kinematics model analytically, the control parameter of each joint actuator can be effectively computed by inverse kinematics, which makes the control problem relatively intuitive.

%Similar to the rigid robot, finding proper actuation parameters for grasping tasks is modeled as finding the optimum solution for an inverse problem where the target goal (w.r.t. pre-defined requirements) should be satisfied. Before that, a precise and effective kinematics model should be established first (i.e. the forward kinematics solution) to predict the shape change under the given control parameters. After comparing existing analytical and numerical solutions to tackle this problem (see \cite{Rigatos09_AMM} for a survey), we chose a geometry-based numerical computing tool \cite{Fang18_ICRA} since the variables used in formulating the grasping task are all geometry-defined (i.e., the tip position, the grasping angle and the curvature diameter defined in Sec.III(a)). This solution can balance the computational cost and the precision of kinematic model.

\subsection{Contribution}

In this paper, we develop an optimization-based motion planning pipeline to compute the proper trajectory and control parameters set to realize the task for soft manipulators. In particular, precise and tight pick-and-place task in a fixed restricted environment with obstacles are studied. As it is based on numerical modeling, our method is general to soft robots with complex shape and can be easily transformed to realize different functions.

Based on~\cite{Langowski20_sciRobot}, the grasping mechanism of soft robot is divided to three categories including mechanical interlocking~\cite{}, friction~\cite{}, and adhesion~\cite{}. In this paper, we mainly focused on conduct the objective of first two grasping behavior in the motion planning process, where the pick-and-place task is studied with setups contains various combination of soft manipulators and grippers.

The contribution of this letter are summarized as follow:
\begin{itemize}
    \item Develop a method for soft robot motion planning based on multi-level optimization. Formulate the effective soft robot pick-and-place task objectives in fixed restricted environment with obstacles.
    \item Conduct the learning scheme for both kinematics and collision avoidance function for soft robot based on data generated from numerical simulation, which enables a fast computing speed of motion planning task.
\end{itemize}

The rest of the paper is organized as follows: Sec. II presents a soft manipulator design and the details of the geometry-based kinematic modeling. After that, the grasping task is separated into three steps and different geometry-oriented objective functions are presented to formulate the inverse control problem. A gradient-based method for solving this inverse problem is also presented in Sec. III. We show the experiment results in Sec. IV to verify the behavior our method and the paper ends with the conclusion and future work discussion in Sec. V. \guoxin{rewrite this in the end of paper preparation.}


